Truly Multi-modal YouTube-8M Video Classification with Video, Audio, and Text

The YouTube-8M video classification challenge requires teams to classify 0.7 million videos into one or more of 4,716 classes. In this Kaggle competition, we placed in the top 3% out of 650 participants using released video and audio features. Beyond that, we extend the original competition by including text information in the classification, making this a truly multi-modal approach with vision, audio and text. The newly introduced text data is termed as YouTube-8M-Text. We present a classification framework for the joint use of text, visual and audio features, and conduct an extensive set of experiments to quantify the benefit that this additional mode brings. The inclusion of text yields state-of-the-art results, e.g. 86.7% GAP on the YouTube-8M-Text validation dataset.

==> eval_metrics.tex <==
\todo{THIS FILE SHOULD NOT BE USED WITHOUT CHECKING THE CONTENTS.}

\subsection{Evaluation Metrics}
The YouTube-8M authors \cite{abu2016youtube} use four metrics to quantify the performance of their models. To facilitate comparison, we report performance using all four metrics. These metrics are:

\begin{enumerate}
  \item \textbf{Global Average Precision (GAP):} GAP is the measure of performance of a model over a dataset. We use the model to predict the $k$ most likely labels of all $m$ examples in the dataset, and then sort the (label, confidence) triplets by confidence score.

  statistic over we evaluate the GAP at k, where k=20, for the predicted scores of our models. If one model totally has N predictions (label/confidence pairs) sorted by its confidence score, then the Global Average Precision is computed as:

where N is the number of final predictions (if there are 20 predictions for each video, then N = 20 * #Videos ), p(i) is the precision, and r(i) is the recall.

Mean Average Precision (mAP): the mAP[1] is computed as the unweighted mean of all the per-class average precisions where the average precision approximates the area under the precision-recall curve.

Hit@k: this is the fraction of test samples that contain at least one of the ground truth labels in the top k predictions[1]. We set k=1 in all experiments.

Precision at equal recall rate (PERR): PERR[1] is defined as the video level annotation precision when the same number of entities per video is retrieved as there are in the ground-truth.
\end{enumerate}


==> figures/kagglerank.tex <==
\begin{table}[t]
\centering
\begin{tabularx}{\columnwidth}{c X c}
\toprule
\textbf{Rank} & \textbf{Team Name} & \textbf{GAP (\%)}
\\ \midrule
   1  & WILLOW & 84.97
\\ 2  & monkeytyping & 84.59
\\ 3  & offline & 84.54
\\ 10 & Samaritan & 83.66
\\ 20 & DeeepVideo & 82.92
\\ \textbf{22} & \textbf{DL2.0 (Our Team)} & \textbf{82.74} 
\\ 50 & n01z3 & 81.50
\\ 100 & lwei & 80.37
\\ 200 & CFB1 & 78.25
\\ \bottomrule
\end{tabularx}
\caption{Ranking Table, 650 teams in total. GAP on held-out test labels reported. }
\label{tab:kagglerank}
\end{table}

==> figures/kagglestruct.tex <==
\newcommand{\kagglestructrules}{\cmidrule(lr){2-4}}

\begin{table*}[!t]
\centering
\begin{tabularx}{.8\linewidth}{rrXc}\toprule
\multicolumn{2}{c}{Model} & Parameters & GAP(\%)
\\ \cmidrule(lr){1-4}
\multirow{2}{*}{Video Level}
   & MOE A & Expert=8  & 79.44 
\\ & MOE B & Expert=32 & 79.76
\\ \cmidrule(lr){1-4}\cmidrule(lr){1-4}
\multirow{4}{*}{Frame Level}
   & DBOF A & Projection=8K, Hidden=1K, E=2, Sample=30 & 79.27
\\ & DBOF B & Projection=16K, Hidden=2K, Expert=16, Sample=60 &	80.18
\\\cmidrule(lr){2-4}
   & LSTM A & Layer=1K, Cell=2, Expert=2  & 80.22
\\ & LSTM B & Layer=512, Cell=4, Expert=4 & 79.30
\\ \cmidrule(lr){1-4}
\multicolumn{2}{c}{\multirow{3}{*}{Model Ensembling}}
     & Average Pooling & \textbf{82.74}
\\ & & Max Pooling	   & 81.56
\\ & & Random Forest   & 78.35
%\\ & & Max Pooling     & 81.56
%\\ & & Random Forest   & 78.35
\\ \bottomrule
\end{tabularx}
\caption{\todo{Caption? Text reference?}}
\label{tab:kaggle}
\end{table*}


==> figures/moe_va.tex <==
\begin{table}
\centering
\begin{tabularx}{\linewidth}{Cccc}
\toprule
& \multicolumn{2}{c}{Feature} & 
\\ Model & Visual & Audio & GAP
\\ \hline
\multirow{3}{*}{Mixture of Experts} & \tick & & 74.17 \\
& & \tick & 45.17 \\
& \tick & \tick & 78.18 \\
\bottomrule
\end{tabularx}
\caption{\todo{Caption? Reference in text?}}
\label{tab:visual_audio}
\end{table}


==> figures/params_text.tex <==
\begin{table*}[h]
\centering
\begin{tabularx}{\linewidth}{cccXc}
\toprule
\multicolumn{2}{c}{Model} & Filter Labels & Parameters & GAP(\%)
\\
\midrule
\multirow{2}{*}{TextCNN}
    &  &  & Filter Widths=(1, 2, ..., 8), Filter Channels=512 & 53.5
    \\
    &  & \tick & Filter Widths=(1, 2, ..., 8), Filter Channels=512 & 41.0
\\
\midrule
\multirow{2}{*}{Keywords}
    &  &  &  & 46.2
    \\
    &  & \tick &  & 38.9
\\
\midrule
\multirow{2}{*}{Unigram}
    & Keywords &  &  & 22.6
    \\
    & Titles &  &  & 19.2
\\
\bottomrule
\end{tabularx}
\caption{Performance of text models with different parameters when evaluating on the validation set.}
\label{tab:params_text}
\end{table*}


==> figures/results_modality.tex <==
\newcommand{\modalityrules}{\cmidrule(lr){1-3}\cmidrule(lr){4-7}}
\begin{table*}[t]
\centering
\begin{tabularx}{0.8\linewidth}{ C  cccc  cccc}
\toprule
 & \multicolumn{4}{c}{Features} & \multicolumn{4}{c}{Performance(\%)}
\\
Model & Visual & Audio & Keyword & Title & GAP & Hit@1 & PERR & mAP
\\ \cmidrule(lr){1-1} \cmidrule(lr){2-5}\cmidrule(lr){6-9}
\multirow{5}{*}{Mixture of Expert} 
& \tick &	\tick & &	&		77.6 &	83.7 &	70.2 &	31.9 \\
& 		\tick & & & 	&	35.8 &	46.4 &	35.9 &	14.5 \\
& 		&	\tick & & 	& 60.7 &	71.0 &	57.8 &	49.5 
\\ \cmidrule(lr){2-5}\cmidrule(lr){6-9}
& \tick &	\tick &	\tick & &		79.6 &	85.9 &	72.8 & 	42.9 \\
& \tick &	\tick &	\tick &	\tick &	\textbf{86.7} &	\textbf{91.5} &	\textbf{80.4} &	\textbf{62.8}
\\ \cmidrule(lr){1-1} \cmidrule(lr){2-5}\cmidrule(lr){6-9}
Model on Kaggle & 	\tick &	\tick & &	&		81.1 &	- &	- &	-\\
\bottomrule
\end{tabularx}
\caption{\todo{Caption, Text Reference}}
\label{tab:results_modality}
\end{table*}



==> figures/results_text.tex <==
\newcommand{\restextrules}{\cmidrule(){1-1}\cmidrule(lr){2-3}\cmidrule(){4-7}}
\begin{table}
\begin{tabularx}{\linewidth}{c cc cccc}\toprule
        \multicolumn{3}{c}{Features} & \multicolumn{4}{c}{Performance}
\\      \small Model &\small  Title &\small  K/w &\small  GAP    &\small  Hit@1   &\small  PERR &\small  mAP
\\ \restextrules \multirow{2}{*}{\shortstack{Exact}}
              & \tick &       &        & .099    &       &       % T
\\            &       & \tick &        & .085    &       &       % K
\\ \restextrules \multirow{3}{*}{\shortstack{Unigram}}
              & \tick &       &        &          &       &       % T
\\            &       & \tick &   .226     &          &       &       % K
\\            & \tick & \tick &        &          &       &       % K
\\ \restextrules \multirow{3}{*}{\shortstack{MOE}}
              & \tick &       & .607   &  .710    & .578  & .495  % T
\\            &       & \tick & .358   &  .464    & .359  & .145  % K
\\            & \tick & \tick & .654   &  .758    & .620  & .500  % TK
\\ \restextrules \multirow{4}{*}{\shortstack{MOE \\+ Video \\+ Audio}}
              &       &       & .776   &  .837    & .702  & .319  % 
\\            & \tick &       & .864   &  .911    & .699  & .627  % T
\\            &       & \tick & .796   &  .859    & .728  & .429  % K
\\            & \tick & \tick & \textbf{.867}
                                       &  .915    & .804  & .628  % TK
\\ \bottomrule
    \end{tabularx}
    \caption{Performance of text classifiers given titles and keywords (K/w for short). This performance is calculated on test set videos that include at least one word that is recognized by our English-only Word2Vec model.}
    \label{tab:results_text}
\end{table}


